Ripple Effects: Robust Norms without Punishment

I propose a novel, tractable model of pro-social norms in large communities with slightly altruistic agents. Agents participate in the norm to influence others to participate in the norm, influencing further agents. A continuum of equilibria sustain the pro-social norm, varying in the distribution of how much agents are influenced by their observations. If agents' effective altruism $\alpha$ is larger than their impatience $1-\delta$, equilibria exist that are robust to a population of bad actors. Greater strategic homogeneity increases the robustness of the norm. Robustness is not improved by increasing the number of observers of each action beyond 1.

==> App/purified.tex <==

\subsection{Purified Model}\label{app:pf.het}
\begin{prop}
    If $\alpha$ is independent of $\theta$ in eq. \ref{eq:pref2}, and $\rho$ is a non-atomic distribution then the unique pPSE is always defect.\footnote{This result is related to the non-purification result of \cite{BMM08}.}
\end{prop}

\begin{proof}
    There exists a pPSE where some agents are willing to cooperate after some history. Because their preference is history independent, they are also willing to cooperate after \textit{any} history. Since $\alpha$ is strictly increasing in $\omega$, there is a unique type $\omega^\ast$ that is indifferent between cooperating and defecting. Every other agent will have a strict best response, and thus will cooperate or defect independent of history. By non-atomicity, $\rho\{\omega^\ast\}=0$, meaning that cooperating or defecting has no effect on the distributions of others' actions. By Property 2 of $\Delta$, agents strictly prefer to defect in such a scenario.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:pure.mono}]
    \textbf{Monotonicity:} Fix a strategy $a$, and let $a_\omega:\theta\mapsto a(\theta,\omega)$ for a fixed $\omega$, and $\Delta\in\mathbb{R}$ be the externality created by this strategy. Since $\alpha$ is increasing, this strategy can be described by a cutoff state $\theta^\ast_\Delta(\omega)$ (decreasing in $\omega$) such that
    \begin{equation*}
        a^{-1}_\omega(C)\ge\theta^\ast_\Delta(\omega)\ge a^{-1}_\omega(D).
    \end{equation*}    
    
    To check the strategy is monotonic, we verify that if an agent cooperates one period and they observe no defections, then they cooperate the next period. By Assumption 1 it is sufficient to check that if an agent cooperates in state $\theta^\ast_\Delta(\omega)$ they will also cooperate in state $\theta^+(C,O\rvert\theta^\ast_\Delta(\omega))$ for any $O\in \mathscr{O}_C$.
    
    Since agents cooperate on-path, $a_\omega(\theta_C)=C$, and $\theta_C\ge \theta^\ast_\Delta(\omega)$ for $\rho$-a.a. $\omega$. If equality holds for a type $\omega$, then monotonicity holds for that type since $\theta^+(C,O\rvert\theta_C)=\theta_C$. 
 
    On the other hand, for types $\omega$ such that $\theta_C>\theta^\ast_\Delta(\omega)$, Assumptions (1,2) ensure $\theta^+(C,O\rvert\theta^\ast_\Delta(\omega))>\theta^\ast_\Delta(\omega)$. 

    \textbf{Recurrence:} Assumption 2 means that there are a finite number of defections that will get an agent to $\theta_D$ starting at any state. If $\theta_D\ge \theta_C$ then we are done. Otherwise, because $\lim \nu_n(\eta)=0$, agents must put positive weight on cooperating in state $\theta_D$, meaning $\theta_D\ge \theta^\ast_\Delta(\omega)$ for a.e $\omega$. By monontonicity of $\eta$, agents then cooperate for every subsequent state if no defections are observed, and stability of $\theta_C$ means that there is a finite number of these cooperations necessary to arrive at $\theta_C$.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:bounds}]
            By Lemma \ref{lem:cont}, $\mu\mapsto \tilde{\Delta}(\mu)$ is continuous over the set $\{\mu\in\Delta\Sigma;\overline{n}(\mu)<1\}$. Thus if $\underline{\Delta}$ is such that $\hat{\Delta}(\underline{\Delta})\ge \underline{\Delta}$ and $\overline{n}(\hat\mu\circ\hat\omega(\underline{\Delta}))<1$, then there exists a fixed point $\Delta^\ast\in[\underline{\Delta}, \hat\Delta(\underline{\Delta})]$ with $\overline{n}(\hat\mu\circ\hat\omega(\Delta^\ast))\le\overline{n}(\hat\mu\circ\hat\omega(\underline{\Delta}))<1$. Moreover $\hat\omega_\infty(\Delta^\ast)<\hat\omega_\infty(\underline\Delta)\le \min\supp{\rho}$.
\end{proof}
\begin{proof}[Proof of Corollary \ref{corr:het.exist}]
    (1) holds since $\Delta<\frac{s_1}{1-\beta\delta}$ can be induced by a strategy that randomizes strictly between $1$TFT and always cooperate, while the induced best response is impulse equivalent to a TFT strategy that puts no weight on always cooperating, (2) $\overline{n}(\hat\mu\circ\hat\omega(\underline{\Delta}))\le\beta\lfloor\frac{1}{\beta}\rfloor \le 1$, (3) is implied since $\hat\omega_\infty(\Delta)\le \min\supp{\rho}$,
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:ceiling}]
    In the first case, decreasing the wealth cap allows the $\overline{\omega}$ type to retain $m$TFT as a best response at the externality $\Delta^\ast$. Thus $\Delta^\ast$ generates the same best response across the population and remains an equilibrium.
    
    The second case only holds if there is a mass of agents at $\overline{\omega}_1=\hat{\omega}_{m-1}(\Delta^\ast)$, and this mass of agents puts some weight on the less reactive strategy $(m-1)$TFT.

    \textbf{Claim:} the externality will be such that the cap-type $\overline{\omega}$ will be willing to randomize between the two strategies $m$TFT and $(m-1)$TFT, ie. $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))=\overline{\omega}$ where $\Delta^\ast(\overline{\omega})$ is the equilibrium externality for the cap $\overline\omega$. (Proof in Appendix \ref{app:pf.het}).

    This claim allows us to calculate
    \begin{subequations}
    \begin{equation}\label{eq:dDelta}
        %\overline{\omega}= \hat\omega_{m-1}(\Delta^\ast)\qquad\Longrightarrow \qquad
        \deriv{\Delta^\ast}{\overline\omega}(\overline\omega_1)=\frac{1}{\hat\omega_{m-1}'(\Delta^\ast_1)}.
    \end{equation}

    Furthermore, if the only atom in our distribution is at the wealth cap $\overline{\omega}$, we can calculate the change in induced externality (defined explicitly in eq. \ref{eq:Delta.hat}):
    \begin{equation}\label{eq:Delta'}
        \hat\Delta'(\Delta^\ast_1)=\frac{\beta(\Delta^\ast_1)^2}{s_1}\bigg(\sum_{n\ge m}^\infty \delta^{n+1}\deriv{\rho}{\omega}(\hat\omega_n)\hat\omega_n'(\Delta)+\delta^{m}\deriv{\overline{p}}{\Delta}\bigg).
    \end{equation}
    \end{subequations}
    Each term in the summation is the change in externality due to agents crossing the threshold from $n$TFT to $(n+1)$TFT --- where $\deriv{\rho}{\omega}(\hat\omega_n)\hat\omega_n'(\Delta^\ast_1)$ is the measure of agents that cross this threshold --- and the second term is the change in externality due to the agents at the cap $\overline{\omega}$ changing how they randomize between strategies.

    Combining eqs. \ref{eq:dDelta} and \ref{eq:Delta'}, we obtain
    \begin{subequations}
    \begin{equation}\label{eq:Delta.omega}
        \deriv{\Delta^\ast}{\overline{\omega}}=\frac{\beta(\Delta^\ast_1)^2}{s_1}\bigg(\sum_{n\ge m}^\infty \delta^{n+1}\deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta^\ast_1)}{\hat\omega_{m-1}'(\Delta^\ast_1)}+\delta^{m}\deriv{\overline{p}}{\overline{\omega}}\bigg).
    \end{equation}

    Similarly we can calculate the change in reproduction rate:
    \begin{equation}\label{eq:n.omega}
        \deriv{\overline{n}}{\overline\omega}=\sum_{n\ge m} \deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta)}{\hat\omega_m'(\Delta)}+\deriv{\overline{p}}{\overline{\omega}}.
    \end{equation}
    \end{subequations}
    Combining eqs. \ref{eq:dDelta}, \ref{eq:Delta.omega}, and \ref{eq:n.omega}, we obtain
    \begin{equation*}
        \deriv{\overline{n}}{\overline{\omega}}=\sum_{n\ge m} (1-\delta^{1+n-m}) \deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta^\ast_1)}{\hat\omega_{m-1}'(\Delta^\ast_1)}+\frac{s_1}{\beta\delta^{m} (\Delta^\ast_1)^2\hat\omega'_{m-1}(\Delta^\ast_1)}.
    \end{equation*}
    Setting this greater than zero and multiplying by the negative quantity $\omega'_{m-1}(\Delta^\ast_1)$ completes the proof.
\end{proof}
\begin{proof}[Proof of Claim in Proposition \ref{prop:ceil}]
        If $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))<\overline{\omega}$ then the cap type $\overline{\omega}$ is playing a weakly less reactive strategy than $m$TFT, likewise all other types are also playing weakly less reactive strategies since other thresholds have decreased. Thus $\hat\Delta(\Delta^\ast(\overline{\omega}))<\Delta^\ast$, contradicting Lemma \ref{lem:bounds}. 

    If $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))>\overline{\omega}$, then there is a discrete jump in $\hat\Delta(\Delta^\ast(\overline\omega))$ as measure $\hat\mu_{m-1}$ of agents now have a strict best response equivalent to $m$TFT rather than their previous strategy of $(m-1)$TFT. As $\overline{\omega}\rightarrow\overline\omega_1$, we then have $\hat\omega_{m-1}(\hat\Delta(\Delta^\ast(\overline\omega)))<\overline{\omega}$.
\end{proof}
\begin{proof}[Proof of Proposition \ref{prop:ceiling}]
    In the first case, decreasing the wealth cap allows the $\overline{\omega}$ type to retain $m$TFT as a best response at the externality $\Delta^\ast$. Thus $\Delta^\ast$ generates the same best response across the population and remains an equilibrium.
    
    The second case only holds if there is a mass of agents at $\overline{\omega}_1=\hat{\omega}_{m-1}(\Delta^\ast)$, and this mass of agents puts some weight on the less reactive strategy $(m-1)$TFT.

    \textbf{Claim:} the externality will be such that the cap-type $\overline{\omega}$ will be willing to randomize between the two strategies $m$TFT and $(m-1)$TFT, ie. $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))=\overline{\omega}$ where $\Delta^\ast(\overline{\omega})$ is the equilibrium externality for the cap $\overline\omega$. (Proof in Appendix \ref{app:pf.het}).

    This claim allows us to calculate
    \begin{subequations}
    \begin{equation}\label{eq:dDelta}
        %\overline{\omega}= \hat\omega_{m-1}(\Delta^\ast)\qquad\Longrightarrow \qquad
        \deriv{\Delta^\ast}{\overline\omega}(\overline\omega_1)=\frac{1}{\hat\omega_{m-1}'(\Delta^\ast_1)}.
    \end{equation}

    Furthermore, if the only atom in our distribution is at the wealth cap $\overline{\omega}$, we can calculate the change in induced externality (defined explicitly in eq. \ref{eq:Delta.hat}):
    \begin{equation}\label{eq:Delta'}
        \hat\Delta'(\Delta^\ast_1)=\frac{\beta(\Delta^\ast_1)^2}{s_1}\bigg(\sum_{n\ge m}^\infty \delta^{n+1}\deriv{\rho}{\omega}(\hat\omega_n)\hat\omega_n'(\Delta)+\delta^{m}\deriv{\overline{p}}{\Delta}\bigg).
    \end{equation}
    \end{subequations}
    Each term in the summation is the change in externality due to agents crossing the threshold from $n$TFT to $(n+1)$TFT --- where $\deriv{\rho}{\omega}(\hat\omega_n)\hat\omega_n'(\Delta^\ast_1)$ is the measure of agents that cross this threshold --- and the second term is the change in externality due to the agents at the cap $\overline{\omega}$ changing how they randomize between strategies.

    Combining eqs. \ref{eq:dDelta} and \ref{eq:Delta'}, we obtain
    \begin{subequations}
    \begin{equation}\label{eq:Delta.omega}
        \deriv{\Delta^\ast}{\overline{\omega}}=\frac{\beta(\Delta^\ast_1)^2}{s_1}\bigg(\sum_{n\ge m}^\infty \delta^{n+1}\deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta^\ast_1)}{\hat\omega_{m-1}'(\Delta^\ast_1)}+\delta^{m}\deriv{\overline{p}}{\overline{\omega}}\bigg).
    \end{equation}

    Similarly we can calculate the change in reproduction rate:
    \begin{equation}\label{eq:n.omega}
        \deriv{\overline{n}}{\overline\omega}=\sum_{n\ge m} \deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta)}{\hat\omega_m'(\Delta)}+\deriv{\overline{p}}{\overline{\omega}}.
    \end{equation}
    \end{subequations}
    Combining eqs. \ref{eq:dDelta}, \ref{eq:Delta.omega}, and \ref{eq:n.omega}, we obtain
    \begin{equation*}
        \deriv{\overline{n}}{\overline{\omega}}=\sum_{n\ge m} (1-\delta^{1+n-m}) \deriv{\rho}{\omega}(\hat\omega_n)\frac{\hat\omega_n'(\Delta^\ast_1)}{\hat\omega_{m-1}'(\Delta^\ast_1)}+\frac{s_1}{\beta\delta^{m} (\Delta^\ast_1)^2\hat\omega'_{m-1}(\Delta^\ast_1)}.
    \end{equation*}
    Setting this greater than zero and multiplying by the negative quantity $\omega'_{m-1}(\Delta^\ast_1)$ completes the proof.
\end{proof}
\begin{proof}[Proof of Claim in Proposition \ref{prop:ceiling}]
        If $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))<\overline{\omega}$ then the cap type $\overline{\omega}$ is playing a weakly less reactive strategy than $m$TFT, likewise all other types are also playing weakly less reactive strategies since other thresholds have decreased. Thus $\hat\Delta(\Delta^\ast(\overline{\omega}))<\Delta^\ast$, contradicting Lemma \ref{lem:bounds}. 

    If $\hat\omega_{m-1}(\Delta^\ast(\overline\omega))>\overline{\omega}$, then there is a discrete jump in $\hat\Delta(\Delta^\ast(\overline\omega))$ as measure $\hat\mu_{m-1}$ of agents now have a strict best response equivalent to $m$TFT rather than their previous strategy of $(m-1)$TFT. As $\overline{\omega}\rightarrow\overline\omega_1$, we then have $\hat\omega_{m-1}(\hat\Delta(\Delta^\ast(\overline\omega)))<\overline{\omega}$.
\end{proof}
